Aura: Privacy-preserving Augmentation to Improve Test Set Diversity in Speech Enhancement

Noise suppression models running in production environments are commonly trained on publicly available datasets. However, this approach leads to regressions due to the lack of training/testing on representative customer data. Moreover, due to privacy reasons, developers cannot listen to customer content. This `ears-off' situation motivates augmenting existing datasets in a privacy-preserving manner. In this paper, we present Aura, a solution to make existing noise suppression test sets more challenging and diverse while being sample efficient. Aura is `ears-off' because it relies on a feature extractor and a metric of speech quality, DNSMOS P.835, both pre-trained on data obtained from public sources. As an application of Aura, we augment the INTERSPEECH 2021 DNS challenge by sampling audio files from a new batch of data of 20K clean speech clips from Librivox mixed with noise clips obtained from AudioSet. Aura makes the existing benchmark test set harder by 0.27 in DNSMOS P.835 OVLR (7%), 0.64 harder in DNSMOS P.835 SIG (16%), increases diversity by 31%, and achieves a 26% improvement in Spearman's rank correlation coefficient (SRCC) compared to random sampling. Finally, we open-source Aura to stimulate research of test set development.

==> TODO.tex <==
TODO:
1. DONE: Description of AEC data we sample from
2. DONE: Do we normalize chi-square? 
3. DONE: Reference for AECMOS
4. WONT WORK: Update code in github page -- I dontthink we can do this unless there is a Python AEC. A quick glance does not yield anything like what we have. 
5. Do we have a AEC benchmark test set with DMOS/chi-squared?
6. DONE:  Do we add number of classes in Table 2? -- Yes. 
7. DONE: Add conf. interval in table 2? +- 0.01
8. DONE: Improve figure 3 (color + fontsize, overall size).
9. Fit text in 4 pages DONE
10. Fit references in 1 page DONE

From Jay:
11. DONE: Can we represent the improvements in relative terms.
E.g. Abstract mentions improvement of 0.17 SIG MOS and 0.42 OVRL MOS. I think it would be good to provide 
one result for NS and AEC in terms of overall to keep it simple and consistent.

12. DONE: CAn you double check the claim of 0.42 OVRL - I believe this is 0.42 in SIG (not OVRL) per table 1

13. DONE: Could we remove the bold higlighting in Table 1 and Table 2 for greedy.
This was distracting to previous reviewers as they were left confused why our method is worse than greedy.
Instead, we should reinforce that we are finding a balance between challenging and diversity.
We should also give an example of why just challenging alone is not good enough by mentioning that 
the same class is over-represented.

14. DONE: The discussion for #clusters is unclear to me. When I see the plot in absolute terms, it conveys to me that 
there is not that much sensitivity to #clusters - should we shot it in relative terms?
For e.g. the difference in relative terms between 0.20 and 0.09 is quite large.
As a reviewer, I would also be confused between #classes coming from the ontology and #clusters coming from 
our internal feature maps. I feel we could explain this in Section 3.3 and again refer to the motivation 
to do this whenever we reference it to avoid confusion between clustering for representation versus evaluation.

XG: I made more explicit that Aura is not sensitive to the number of clusters. And I added some language in section 3.3 and this section on using clusters as a soft ontology. 

15. Can we make the conclusion stronger and mention that this method is being used to test/evaluate new production models for NS and AEC.

16. CAn we run Grammarly? I found couple of instances in the Abstract so would be great to do it for the whole file.
 







